Fast Arithmetic Hardware Library For RLWE-Based Homomorphic Encryption

In this work, we propose an open-source, first-of-its-kind, arithmetic hardware library with a focus on accelerating the arithmetic operations involved in Ring Learning with Error (RLWE)-based somewhat homomorphic encryption (SHE). We design and implement a hardware accelerator consisting of submodules like Residue Number System (RNS), Chinese Remainder Theorem (CRT), NTT-based polynomial multiplication, modulo inverse, modulo reduction, and all the other polynomial and scalar operations involved in SHE. For all of these operations, wherever possible, we include a hardware-cost efficient serial and a fast parallel implementation in the library. A modular and parameterized design approach helps in easy customization and also provides flexibility to extend these operations for use in most homomorphic encryption applications that fit well into emerging FPGA-equipped cloud architectures. Using the submodules from the library, we prototype a hardware accelerator on FPGA. The evaluation of this hardware accelerator shows a speed up of approximately 4200x and 2950x to evaluate a homomorphic multiplication and addition respectively when compared to an existing software implementation.

==> Makefile <==
# Add a list of home-made EPS figures here.
PDFFIGURES=figs/arch_pipeline.pdf figs/arch_icswitch.pdf

.SUFFIXES: .fig .eps .ps .dvi .bbl .bib .tex .pdf

FIGURES=${wildcard *.fig}
EPSFIGFILES=${FIGURES:.fig=.eps}
TEXFILES=*.tex

all: pdf   

force: rmdone all

dvi: paper.dvi

xdvi: paper.dvi
	xdvi paper.dvi

gv: paper.ps
	gv paper.ps

ps: paper.ps 

pdf: paper.pdf

rmdone:
	rm -f done.flag

done.flag:
	touch done.flag

printerrors:
	@echo "*****************************"; \
	echo Overview of typeset warnings: ; \
        echo "****************************"; \
	grep "Underfull" paper.log; \
	grep "Overfull" paper.log; \
	echo ; \
        echo "***************************"; \
	echo Overview of latex warnings: ; \
        echo "***************************"; \
	grep "LaTeX Warning" paper.log; \
        echo "***************************"; \
	echo ; \
        echo "***************************"; \
	echo Overview of bibtex warnings: ; \
        echo "***************************"; \
        grep ^Warning-- paper.blg; \
	echo "***************************"; \
	echo ; \
        echo "*************************"; \
	echo Overview of latex errors: ; \
        echo "*************************"; \
	grep "^!" paper.log; \
        echo "*************************"; \
	echo

paper.bbl: references.bib $(TEXFILES) Makefile done.flag
	pdflatex -interaction=batchmode paper.tex || true
	rm -f $*.pdf
	bibtex -terse $*

paper.pdf: $(TEXFILES) $(PDFFIGFILES) paper.bbl Makefile done.flag
	@echo Running latex once.; \
	while ( pdflatex -interaction=nonstopmode paper.tex; grep Rerun paper.log ) ; do \
          echo; \
          echo "*********************************"; \
          echo "*********************************"; \
          echo Reruning to complete compilation.; \
          echo "*********************************"; \
          echo "*********************************"; \
	done; \
        echo "***************************"; \
	echo DVI file generated.; \
        echo "***************************"; \
	echo ; \
	make printerrors 
			
clean:
	rm -f *.lof *.lot *.pfg *~ *.aux *.dvi *.blg *.log *.bbl $(EPSFIGFILES) *.bak paper.ps paper.pdf *.toc *.swp done.flag




==> Sections/GCD.tex <==
\subsection{GCD}
%\vspace{-0.1in}
The largest positive integer that divides two or more given integers is known as the greatest common divisor, GCD, of those integers. Mathematically, $gcd(a,b)$ where $a$ and $b$ are not both zero, may be defined as the smallest positive integer $d$ that can be written as $d = a \cdot x\ + b \cdot y$, where $x$ and $y$ are integers. For our implementation purposes, we need to check if two numbers are relatively prime or not by computing the GCD. We know that two numbers are coprime if their GCD equals $1$, which can also be written as $1 = a \cdot x\ + b \cdot y$.  

\subsubsection{Classic Euclidean Method}
%\vspace{-0.1in}
Algorithm \ref{alg:CEAD} shows the way GCD is computed using the classic Euclidean method (aka the long division method). This algorithm computes GCD by recursively dividing the larger number by the smaller number. After each division, the remainder replaces the smaller number involved in the division process. The time complexity of this algorithm is $O(log(min(a, b)))$.       

\begin{algorithm}
	\footnotesize
	\SetCommentSty{\textit}
	\nonl Let $a, b \in \mathbb{Z}_q[x]/\langle f(x) \rangle$ and $a \geq b$. \\

	\nonl \DontPrintSemicolon 	\;	
	\nonl  \textbf{gcd(a, b)} \\
	\If{$a \% b == 0$}
	{\textbf{Return} $b$ as $\langle gcd(a,b) \rangle$.}	
	\Else
	{\textbf{Return} $gcd(b, a \% b)$.}	
	
	\caption{Classic Euclidean Algorithm by Division}
	\label{alg:CEAD}
\end{algorithm}

Division operations are very expensive to implement on FPGA, but we still implement this algorithm so as to evaluate its associated hardware cost and performance. The hardware implementation is shown in Figure \ref{fig:GCD}. We also implement this algorithm with our modified Barrett reduction to see its influence on the hardware cost. We will discuss it later, in Section \ref{Perf}.

\begin{figure*}[!t]
	\begin{center}
		\includegraphics[width=5.5in]{Figures/GCD.pdf} 
		%\vspace{-0.15in}
	\end{center}
	\caption{\small Hardware implementation of different methods to compute GCD: \textit{Classic Euclidean method}, \textit{Subtraction method}, and \textit{Binary method}.} 
	\label{fig:GCD}
	%\vspace{-0.15in}
\end{figure*}

\subsubsection{Subtraction Method}
%\vspace{-0.1in}
Another classic way of computing GCD is via recursive subtraction, wherein we recursively subtract the smaller integer from the larger integer as seen in Algorithm \ref{alg:CEAS}.    

\begin{algorithm}
	\footnotesize
	\SetCommentSty{\textit}
	\nonl Let $a, b \in \mathbb{Z}_q[x]/\langle f(x) \rangle$. \\

	\nonl \DontPrintSemicolon 	\;	
	\nonl  \textbf{gcd(a, b)} \\
	\If{$a == b$}
	{\textbf{Return} $a$ as $\langle gcd(a,b) \rangle$.}	
	\If{$a > b$}
	{\textbf{Return} $gcd(a-b, b)$.}	
	\Else
	{\textbf{Return} $gcd(a, b-a)$.}	
	
	\caption{Euclidean Algorithm by Subtraction}
	\label{alg:CEAS}
	%\vspace{-0.05in}
\end{algorithm}

While the implementation of this algorithm is straight-forward and reduces the hardware cost significantly, the time complexity is higher than the previous algorithm involving divisions. The number of steps are linear, and so the worst case time complexity is $O(max(a,b))$. The hardware circuit is also shown in Figure \ref{fig:GCD}. 

\subsubsection{Binary Euclidean Method} 
%\vspace{-0.1in}
The binary Euclidean method is customized specifically for large integers and works best when all the involved arithmetic operations cannot be done in constant time. Due to the binary representation, operations are performed in linear time based on the length of the binary representation, even for very big integers. As shown in Algorithm \ref{alg:EB}, the GCD is computed with a divide and conquer approach using only subtraction, shift operations, and parity checking. The time complexity of this algorithm is $O(log(a+b))$. The hardware implementation for this algorithm is shown in the Figure \ref{fig:GCD}.     

\begin{algorithm}
	\footnotesize
	\SetCommentSty{\textit}
	\nonl Let $a, b \in \mathbb{Z}_q[x]/\langle f(x) \rangle$. \\

	\nonl \DontPrintSemicolon 	\;	
	\nonl  \textbf{gcd(a, b, res)} \\
	\If{$a == b$}
	{\textbf{Return} $res * a$ as $\langle gcd(a,b) \rangle$.}	
	\ElseIf{$a \% 2 == 0$ and $b \% 2 == 0$}
	{\textbf{Return} $gcd(a/2, b/2, 2*res)$.}
	\ElseIf{$a \% 2 == 0$}
	{\textbf{Return} $gcd(a/2, b, res)$.}
	\ElseIf{$b \% 2 == 0$}
	{\textbf{Return} $gcd(a, b/2, res)$.}
	\ElseIf{$a > b$}
	{\textbf{Return} $gcd(a-b, b, res)$.}
	\Else
	{\textbf{Return} $gcd(a, b-a, res)$.}	
	
	\caption{Binary Euclidean Algorithm}
	\label{alg:EB}
\end{algorithm}

 


